Correct Is Not Enough: Training Reasoning Planners with Executor-Grounded Rewards

Reinforcement learning with verifiable rewards has become a common way to improve explicit reasoning in large language models, but final-answer correctness alone does not reveal whether the reasoning trace is faithful, reliable, or useful to the model that consumes it. This outcome-only signal can reinforce traces that are right for the wrong reasons, overstate reasoning gains by rewarding shortcuts, and propagate flawed intermediate states in multi-step systems. To this end, we propose TraceLift, a planner-executor training framework that treats reasoning as a consumable intermediate artifact. During planner training, the planner emits tagged reasoning. A frozen executor turns this reasoning into the final artifact for verifier feedback, while an executor-grounded reward shapes the intermediate trace. This reward multiplies a rubric-based Reasoning Reward Model (RM) score by measured uplift on the same frozen executor, crediting traces that are both high-quality and useful. To make reasoning quality directly learnable, we introduce TRACELIFT-GROUPS, a rubric-annotated reason-only dataset built from math and code seed problems. Each example is a same-problem group containing a high-quality reference trace and multiple plausible flawed traces with localized perturbations that reduce reasoning quality or solution support while preserving task relevance. Extensive experiments on code and math benchmarks show that this executor-grounded reasoning reward improves the two-stage planner-executor system over execution-only training, suggesting that reasoning supervision should evaluate not only whether a trace looks good, but also whether it helps the model that consumes it. Our code is available at: https://github.com/MasaiahHan/TraceLift

==> figures/latex_includes.tex <==
% Auto-generated by figures/gen_figures.py.
% Numeric tables are parsed from ../../exp_rm.md.
% Tables require \usepackage{booktabs}. The TikZ method figure requires
% \usepackage{tikz} and \usetikzlibrary{arrows.meta,positioning,fit,calc}.

\input{figures/table_code_two_stage_aggregate.tex}

\input{figures/table_math_total_two_stage_direct.tex}

\input{figures/table_rollout_n_ablation.tex}

% Optional per-dataset table for the Qwen2.5 full fine-tuning code setting:
% \input{figures/table_code_qwen25_full_per_dataset.tex}

% Method pipeline TikZ snippet:
\input{figures/fig_method_pipeline_tikz.tex}


==> figures/table_code_qwen25_full_per_dataset.tex <==
\begin{table}[t]
\centering
\caption{Qwen2.5-7B full fine-tuning code two-stage results.}
\label{tab:code-qwen25-full-per-dataset}
\begin{tabular}{lrrrr}
\toprule
Dataset & $N$ & Base & Exec-only Full & \modelname{} Full \\
\midrule
HumanEval & 164 & 113 / 68.90\% & 121 / 73.78\% & 126 / 76.83\% \\
HumanEvalPlus & 164 & 99 / 60.37\% & 112 / 68.29\% & 115 / 70.12\% \\
MBPP-full (500) & 500 & 290 / 58.00\% & 305 / 61.00\% & 318 / 63.60\% \\
LiveCodeBench (public) & 400 & 118 / 29.50\% & 173 / 43.25\% & 181 / 45.25\% \\
\bottomrule
\end{tabular}
\end{table}


==> figures/table_code_two_stage_aggregate.tex <==
\begin{table}[t]
\centering
\caption{Code two-stage pass@1. Aggregates are micro-averages over HumanEval, HumanEvalPlus, MBPP-full, and LiveCodeBench public tests; $\Delta$ is \modelname{} minus Exec-only.}
\label{tab:code-two-stage-aggregate}
\begin{tabular}{lrrrr}
\toprule
Model / setting & Base & Exec-only & \modelname{} & $\Delta$ \\
\midrule
Qwen2.5-7B & 50.49\% & 52.28\% & 54.89\% & 2.61 pp \\
Llama3.1-8B & 25.81\% & 32.49\% & 34.45\% & 1.95 pp \\
Qwen3-4B & 64.74\% & 65.88\% & 68.32\% & 2.44 pp \\
Qwen2.5-7B Full FT & 50.49\% & 57.90\% & 60.26\% & 2.36 pp \\
\bottomrule
\end{tabular}
\end{table}


==> figures/table_math_total_two_stage_direct.tex <==
\begin{table}[t]
\centering
\caption{Math total pass@1 under two-stage planner-executor evaluation and direct self-solving, using the Total rows in exp\_rm.md.}
\label{tab:math-total-two-stage-direct}
\begin{tabular}{llrrrr}
\toprule
Model & Protocol & Base & Exec-only & \modelname{} & $\Delta$ \\
\midrule
Qwen2.5-7B & two-stage & 46.51\% & 64.72\% & 69.23\% & 4.51 pp \\
Qwen2.5-7B & direct & 46.51\% & 65.62\% & 70.19\% & 4.57 pp \\
Llama3.1-8B & two-stage & 12.74\% & 22.13\% & 23.82\% & 1.69 pp \\
Llama3.1-8B & direct & 12.74\% & 22.19\% & 22.86\% & 0.67 pp \\
Qwen3-4B & two-stage & 71.20\% & 71.50\% & 72.34\% & 0.84 pp \\
Qwen3-4B & direct & 71.20\% & 71.93\% & 72.25\% & 0.32 pp \\
\bottomrule
\end{tabular}
\end{table}


==> figures/table_rollout_n_ablation.tex <==
\begin{table}[t]
\centering
\caption{Executor comparison-count ablation for estimating uplift in Qwen2.5-7B code \modelname{}.}
\label{tab:rollout-n-ablation}
\begin{tabular}{lrrrr}
\toprule
Dataset & $N$ & $n=1$ & $n=3$ & $n=5$ \\
\midrule
HumanEval & 164 & 68.29\% & 72.56\% & 67.07\% \\
HumanEvalPlus & 164 & 63.41\% & 64.02\% & 60.37\% \\
MBPP-full (500) & 500 & 60.80\% & 61.20\% & 60.40\% \\
LiveCodeBench (public) & 400 & 35.00\% & 36.00\% & 35.50\% \\
Micro-average & 1228 & 53.75\% & 54.89\% & 53.18\% \\
\bottomrule
\end{tabular}
\end{table}


==> sections/limitations.tex <==
\section{Analysis, Limitations, and Scope}
\label{sec:limitations}

The current evidence supports a controlled planner-executor claim: \modelname{} improves a fixed two-stage system over execution-only RL under the same evaluation chain. It does not support a claim of direct standalone state-of-the-art code or math performance. In our main results, the policy generates reasoning, the frozen executor generates the final artifact, and the reported score belongs to that two-stage system. These scores should therefore not be compared directly to leaderboards where one model produces the final answer or code.

\paragraph{Reward components.}
Uplift and the end-to-end verifier anchor are part of the \modelname{} reward design, but the current experiments do not yet prove that each component is necessary. The completed rollout-count ablation shows that $n=3$ is the best setting among $n=1,3,5$ for the current Qwen2.5-7B code runs, but this does not isolate uplift itself. The No-uplift ablation and the RM-uplift-only/no-end-to-end-anchor ablation remain pending in this draft. Until those experiments are complete, the safe conclusion is that the combined reward is effective in the tested recipe, not that every component has been causally isolated.

\paragraph{Mechanism diagnostics.}
We have not yet reported correlations among RM score, executor utility, reasoning reward, and final pass/fail. We also lack win/loss flip analysis comparing Exec-only and \modelname{} on the same examples, and we have not controlled for reasoning length or formatting artifacts. These analyses are needed to rule out superficial explanations such as the planner learning longer traces, better tag compliance, or styles preferred by the executor independently of reasoning quality.

\paragraph{Data audit.}
The data construction examples show that problem-level groups can contain meaningful targeted negatives, including wrong algorithms, incorrect invariants, missing edge cases, off-by-one errors, wrong operations, dropped cases, unsupported jumps, and verbose content-free reasoning. However, the current draft does not yet report full dataset scale, negative-type distributions, leakage rates, judge consistency, train/evaluation overlap checks, or manual audit statistics. These details are required before a submission version can make a strong data-quality claim.

\paragraph{Evaluation uncertainty and scope.}
The current tables are single-run summaries without confidence intervals, paired bootstrap tests, or sign tests over matched examples. The LiveCodeBench results use public/local tests, and MBPP-full uses a 500-example split rather than the EvalPlus leaderboard protocol. Finally, while the method formulation naturally extends to tool-use decisions by treating the next action as the executor artifact, tool-use is not experimentally validated in this draft.

